ATMPlace: Analytical Thermo-Mechanical-Aware Placement Framework for 2.5D-IC

Rising demand in AI and automotive applications is accelerating 2.5D IC adoption, with multiple chiplets tightly placed to enable high-speed interconnects and heterogeneous integration. As chiplet counts grow, traditional placement tools, limited by poor scalability and reliance on slow simulations, must evolve beyond wirelength minimization to address thermal and mechanical reliability, critical challenges in heterogeneous integration. In this paper, we present ATMPlace, the first analytical placer for 2.5D ICs that jointly optimizes wirelength, peak temperature, and operational warpage using physics-based compact models. It generates Pareto optimal placements for systems with dozens of chiplets. Experimental results demonstrate superior performance: 146 percent and 52 percent geometric mean wirelength improvement over TAP 2.5D and TACPlace, respectively, with 3 to 13 percent lower temperature and 5 to 27 percent less warpage, all achieved approximately 10 times faster. The proposed framework is general and can be extended to enable fast, scalable, and reliable design exploration for next-generation 2.5D systems.

==> Textlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\iffalse
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=35pt, bottom=45pt, 
    left=40pt, right=40pt, 
    %inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\fi
\iftrue
\geometry{twoside=true, head=13pt,
paperwidth=8.5in, paperheight=11in,
includeheadfoot, columnsep=2pc,
top=57pt, bottom=73pt, inner=54pt, outer=54pt,
marginparwidth=2pc,heightrounded
}%
\fi
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\let\Bbbk\relax % redefined in newtxmath.sty
\newcommand\hmmax{0}
\newcommand\bmmax{0}
% \usepackage{amssymb}
% \usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
%\usepackage{siunitx}
%\sisetup{product-units = single}
% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
\newcommand{\m}[1]{\mathbf{#1}}
\newcommand{\mx}{\m{x}}
\newcommand{\my}{\m{y}}
\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}



% yuxiang setting

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage{biblatex}
% \usepackage[a4paper, total={184mm,239mm}]{geometry}
% % \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
% %     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\graphicspath{{./Images/}}
\usepackage{color}
\usepackage{xcolor}
\usepackage{threeparttable}
\usepackage{utfsym}
\usepackage{url}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{subfig}
\usepackage{float}
\usepackage{algorithm}
\usepackage{cleveref}
\usepackage{hyperref}
\usepackage[export]{adjustbox}
% \usepackage[margin = 3.5cm]{geometry}     % avoid `overfull \hbox' warning
\usepackage[tableposition = top]{caption} % captions
\usepackage{booktabs}                     % horizontal lines in tabless
\usepackage[per-mode = symbol]{siunitx}   % physical quantities and SI units
\usepackage{colortbl,booktabs}
\usepackage{multicol}
\usepackage{multirow} 
\usepackage{multirow, makecell, caption}
\usepackage{diagbox}

\usepackage{booktabs}
% \usepackage{ThreePartTable} 
\usepackage{tabu}
\usepackage{tabularx}
\usepackage{rotating}
\usepackage{supertabular}
\usepackage{tikz}
\usepackage{hhline}
\usepackage{longtable}
\usepackage{svg}
\usepackage{rotating}
\usepackage{xcolor}
\usepackage{bbding}
% \usepackage[fontsize=9pt]{fontsize}

\geometry{twoside=true, head=13pt,
paperwidth=8.5in, paperheight=11in,
includeheadfoot, columnsep=2pc,
top=30pt, bottom=50pt, inner=42pt, outer=42pt,
marginparwidth=2pc,heightrounded
}%
 % \addbibresource{./Ref/bib.bib}



==> Textlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subfig}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command


\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}


% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%



